Minimal central slices of the regular simplex

We prove that minimal-volume hyperplane sections of the regular simplex through its centroid are parallel to a facet. The proof combines variational methods with Fourier-analytic techniques and zero-diminishing arguments to show that every critical normal vector has at most three distinct non-zero coordinates. Analysis of the two- and three-value cases then yields the sharp lower bound.

==> references.tex <==
\begin{biblist}

\bib{BPg25}{arXiv}{
    title={Sharp inequalities for symmetric polynomials, Hunter's conjecture, and moments of exponential random variables},
    author={Brazitikos, Silouanos},
    author={Pandis, Christos},
    archivePrefix={arXiv preprint },
    year={2025},
    eprint={2512.12254}
}

\bib{BPg26}{arXiv}{
	title={Restricted Hyperplane Sections of the Cross-Polytope and the Simplex},
	author={Brazitikos, Silouanos},
    author={Pandis, Christos},
	archivePrefix={arXiv preprint},
	year={2026},%-7-5
	eprint={2606.07163}	
}

\bib{Brz}{article}{
	title={Volume estimates for sections of certain convex bodies},
	author={Brzezinski, Patryk},
	journal={Math. Nachr.},
	volume={286},
	number={17--18},
	pages={1726--1743},
	date={2013}
}

\bib{DirksenD}{thesis}{
	date={2015-12},
	author={Dirksen, Hauke},
	organization={Christian Albrecht University of Kiel},
	subtitle={Volume Formulas and Estimates},
	title={Sections of Simplices and Cylinders},
	type={PhD thesis},
	note={Under the supervision of H. König}
}				

\bib{Dirksen}{article}{
	journal={Math. Nachr.},
	volume={290},
	number={16},
	pages={2567--2584},
	date={2017},
	title={Sections of the regular simplex -- Volume formulas and estimates},
	author={Dirksen, Hauke}
}	

\bib{Filli}{article}{
	author={Filliman, Paul},
	title={The volume of duals and sections of polytopes},
	journal={Mathematika},
	date={1992},
	volume={39},
	pages={67--80},
	number={1}
}

\bib{Fradelizi}{article}{
	author={Fradelizi, Matthieu},
	title={Hyperplane sections of convex bodies in isotropic position},
	journal={Beitr\"age Algebra Geom.},
	volume={40},
	date={1999},
	number={1},
	pages={163--183},
	issn={0138-4821},
	%review={\MR{1678528}},
}
			
\bib{KKönyv}{book}{
	author={Koldobsky, Alexander},
	title={Fourier Analysis in Convex Geometry},
	date={2005},
	volume={116},
	series={Mathematical Surveys and Monographs},
	isbn={0-8218-3787-7},
	publisher={American Mathematical Society}
}

\bib{König21}{article}{
	author={K\"onig, Hermann},
	title={Non-central sections of the simplex, the cross-polytope and the cube},
	journal={Adv. Math.},
	volume={376},
	date={2021},
	pages={Paper No. 107458, 35},
	issn={0001-8708},
	%review={\MR{4178930}},
	%doi={10.1016/j.aim.2020.107458},
}

\bib{König23}{article}{
	title={Non-central sections of the regular n-simplex},
	author={K{\"o}nig, Hermann},
	journal={Pure Appl. Funct. Anal.},
	volume={10},
	number={5},
	pages={1287--1321},
	date={2025}
}

\bib{Laguerre}{book}{
	author={Laguerre, Edmond},
	title={\OE uvres de Laguerre},
	subtitle={Publiées sous les auspices de l'Académie des sciences},
	language={French},
	date={1972},
	edition={2},
	publisher={Chelsea Pub. Co},
	part={1. Algèbre. Calcul intégral}
}

\bib{MRTT}{article}{
    author={Melbourne, James},
    author={Roysdon, Michael},
    author={Tang, Colin},
    author={Tkocz, Tomasz},
    title={From simplex slicing to sharp reverse Hölder inequalities},
    journal={J. London Math. Soc.},
    volume={113},
    number={3},
    pages={e70461},
    date={2026}}
		
\bib{TN-survey}{article}{
	title={Extremal sections and projections of certain convex bodies: a survey},
	%ISBN={9783110775389},
	%url={http://dx.doi.org/10.1515/9783110775389-008},
	%DOI={10.1515/9783110775389-008},
	book={
		title={Harmonic Analysis and Convexity},
		editor={Koldobsky, Alexander},
		editor={Volberg, Alexander},
		volume={9},
		publisher={De Gruyter},
		isbn={978-3-11-077538-9},
		address={Berlin}
	},
	author={Nayar, Piotr},
	author={Tkocz, Tomasz},
	year={2023},
	%month=jul, 
	pages={343–390}
}

\bib{Parodi1}{article}{
	author={Parodi, Maurice},
	title={Sur quelques applications d'un th\'eor\`eme de Laguerre-Polya},
	language={French},
	journal={C. R. Acad. Sci. Paris},
	volume={231},
	date={1950},
	pages={889--890}
	%issn={0001-4036},
	%review={\MR{0037952}},
}

\bib{Parodi2}{article}{
	author={Parodi, Maurice},
	title={Sur quelques nouvelles cons\'equences d'un th\'eor\`eme de Laguerre},
	language={French},
	journal={Bull. Sci. Math. (2)},
	volume={75},
	date={1951},
	pages={41--47},
	issn={0007-4497}
}

\bib{Pólya}{article}{
	author={Pólya, György},
	title={Sur un théro\`eme de Laguerre},
	language={French},
	book={
		title={Comptes rendus hebdomadaires des s{\'e}ances de l'Acad{\'e}mie des sciences},
		note={Issued by the permanent secretaries of the Acad{\'e}mie des sciences},
		volume={156},
		publisher={Gauthier-Villars},
		address={Paris}
	},
	date={1913},
	pages={996--999},
	note = {Available at \url{https://www.biodiversitylibrary.org/item/31588\#page/1002/mode/1up}}
}

\bib{Tang}{article}{
	author={Tang, Colin},
	title={Simplex slicing: an asymptotically-sharp lower bound},
	journal={Adv. Math.},
	volume={451},
	date={2024},
	pages={Paper No. 109784, 25},
	issn={0001-8708},
	%review={\MR{4761953}},
	%doi={10.1016/j.aim.2024.109784},
}
		
\bib{Webb}{article}{
	journal={Geom. Dedicata},
	author={Webb, Simon P.},
	title={Central Slices of the Regular Simplex},
	volume={61},
	pages={19--28},
	date={1996},
	number={1}
}
		
\bib{WebbD}{thesis}{
	author={Webb, Simon P.},
	title={Central Slices of the Regular Simplex},
	type={PhD Thesis},
	date={1996},
	organization={University College London},
	note={Under the supervision of K. Ball}
}
	
\end{biblist}
